FastCLIP: A Suite of Optimization Techniques to Accelerate CLIP Training with Limited Resources

Existing studies of training state-of-the-art Contrastive Language-Image Pretraining (CLIP) models on large-scale data involve hundreds of or even thousands of GPUs due to the requirement of a large batch size. However, such a large amount of resources is not accessible to most people. While advanced compositional optimization techniques for optimizing global contrastive losses have been demonstrated effective for removing the requirement of large batch size, their performance on large-scale data remains underexplored and not optimized. To bridge the gap, this paper explores several aspects of CLIP training with limited resources (e.g., up to tens of GPUs). First, we introduce FastCLIP, a general CLIP training framework built on advanced compositional optimization techniques while designed and optimized for the distributed setting. Our framework is equipped with an efficient gradient reduction strategy to reduce communication overhead. Second, to further boost training efficiency, we investigate three components of the framework from an optimization perspective: the schedule of the inner learning rate, the update rules of the temperature parameter and the model parameters, respectively. Experiments on different strategies for each component shed light on how to conduct CLIP training more efficiently. Finally, we benchmark the performance of FastCLIP and the state-of-the-art training baseline (OpenCLIP) on different compute scales up to 32 GPUs on 8 nodes, and three data scales ranging from 2.7 million, 9.1 million to 315 million image-text pairs to demonstrate the significant improvement of FastCLIP in the resource-limited setting. We release the code of FastCLIP at https://github.com/Optimization-AI/fast_clip .

==> floats/fig_performance.tex <==
\begin{figure}[t]
    \centering
    \if\adjustspaceneurips1
        \vspace{-10pt}
    \fi
    \includegraphics[width=0.25\textwidth]{./figs/in_variants_legend.pdf}
    \if\adjustspaceneurips1
        \vspace{-2pt}
    \fi

    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/in_variants_cc3m_openclip_fastclipv3.png}
        \caption{IN \& Variants, Medium}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/retrieval_cc3m_openclip_fastclipv3.png}
        \caption{Retrieval, Medium}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/in_variants_cc12m_openclip_fastclipv3.png}
        \caption{IN \& Variants, Large}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/retrieval_cc12m_openclip_fastclipv3.png}
        \caption{Retrieval, Large}
    \end{subfigure}
    \caption{Comparison between OpenCLIP and FastCLIP-v3. The numbers in between represent the improvement of FastCLIP-v3 over OpenCLIP.
    }
    \label{fig:performance_nodes}
\end{figure}


==> floats/fig_time.tex <==
\begin{figure}[t]
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{./figs/time_legend.pdf}
    \end{subfigure}

    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/time_cc3m_pure_comm.pdf}
        \caption{Total, Medium}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/time_cc12m_pure_comm.pdf}
        \caption{Total, Large}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.233\textwidth}
        \includegraphics[width=\textwidth]{./figs/time_cc3m_comm.pdf}
        \caption{Comm., Medium}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{./figs/time_cc12m_comm.pdf}
        \caption{Comm., Large}
    \end{subfigure}
    \caption{Comparison of per-iteration running time (ms) between OpenCLIP and FastCLIP.
    Each bar in (a), (b) is divided into (top to bottom): computation, communication, and others. Each bar in (c), (d) is divided into  (top to bottom): communication-computation overlap and pure communication.
    }
    \label{fig:time_nodes}

    \vspace*{0.05in}
    \begin{subfigure}{\textwidth}
        \begin{minipage}[c]{.33\textwidth}
            \centering
            \hspace{-18pt}
            \includegraphics[width=0.7\textwidth]{./figs/in_variants_legend.pdf}
            \vspace{-6pt}
        \end{minipage}
        \hspace{8pt}
        \begin{minipage}[c]{.66\textwidth}
            \centering
            \includegraphics[width=0.9\textwidth]{./figs/speedup_legend.pdf}
        \end{minipage}
    \end{subfigure}
    \if\adjustspaceneurips1
        \vspace{-10pt}
    \fi

    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{./figs/in_laion300m_240904.pdf}
        \caption{ImageNet1k Top1, xLarge}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{./figs/speedup_cc3m.pdf}
        \caption{Speedup, Medium}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{./figs/speedup_cc12m.pdf}
        \caption{Speedup, Large}
    \end{subfigure}

    \caption{Subfigure (a) presents the ImageNet-1k Top1 accuracy curve of OpenCLIP and FastCLIP-v3 in the xLarge-scale setting, with numbers denoting the improvement. Subfigures (b), (c) present the speedup of different algorithms in the medium and large-scale settings, respectively.}

    % \vspace*{0.05in}
    % \includegraphics[width=0.6\textwidth]{./figs/speedup_legend.pdf}

    % \begin{subfigure}{\textwidth}
    %     \centering
    %     \begin{minipage}[c]{.28\textwidth}
    %         \centering
    %         \includegraphics[width=\textwidth]{./figs/speedup_cc3m.pdf}
    %         \caption{Medium}
    %     \end{minipage}
    %     \hspace{30pt}
    %     \begin{minipage}[c]{.28\textwidth}
    %         \centering
    %         \includegraphics[width=\textwidth]{./figs/speedup_cc12m.pdf}
    %         \caption{Large}
    %     \end{minipage}
    % \end{subfigure}

    % \caption{Speedup of different algorithms in the medium and large-scale settings.}
    \label{fig:sped}
\end{figure}


==> floats/tab_components_large.tex <==
{
% \renewcommand{\arraystretch}{1.1}
\definecolor{shaded}{gray}{0.93}
\begin{table}[t]
    \caption{Performance of different inner LR schedules. \colorbox{shaded}{Shaded} algorithms use the cosine schedule, while the others use the constant schedule. Improvement denotes the absolute difference between two algorithms on the three metrics. \(^*\): v3 (Const. \(\gamma\)) denotes FastCLIP-v3 with constant \(\gamma\) schedule.}
    % \begin{widepage}
        \centering
       \resizebox{0.9\columnwidth}{!}{ \begin{tabular}{cccccc}
            \toprule
            Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants              & \textit{Improvement} \\
            \midrule
                                    & SogCLR                          & 29.91 (0.23)          & 30.16 (0.36)                & 22.98 (0.07) &  \\
            \rowcolor{shaded}
            \cellcolor{white}        & FastCLIP-v1                     & \textbf{30.65} (0.11) & \textbf{32.66} (0.12)       & \textbf{24.26} (0.06) & \cellcolor{white} \multirow{-2}{*}{\textit{0.74, 2.50, 1.28}} \\
            \cline{2-6}
                                    & iSogCLR                         & 30.32 (0.18)          & 30.27 (0.41)                & 24.96 (0.09) & \\
            \rowcolor{shaded}
            \cellcolor{white}        & FastCLIP-v2                     & \textbf{30.94} (0.20) & \textbf{31.84} (0.17)       & \textbf{25.52} (0.17) & \cellcolor{white} \multirow{-2}{*}{\textit{0.62, 1.57, 0.56}} \\
            \cline{2-6}
                                    & v3 (Const. \(\gamma\))\(^*\) & 29.46 (0.39)          & 30.33 (0.58)                & 23.69 (0.09) & \\
            \rowcolor{shaded}
            \cellcolor{white} \multirow{-6}{*}{Large} & FastCLIP-v3                     & \textbf{31.60} (0.46) & \textbf{34.88} (0.28)       & \textbf{24.78} (0.28) & \cellcolor{white} \multirow{-2}{*}{\textit{2.14, 4.55, 1.09}} \\
            \bottomrule
        \end{tabular}}
    % \end{widepage}
    \label{tab:gamma}

\vspace*{0.05in}
    \centering
    \caption{Performance of different temperature parameter updates.}
    \begin{tabular}{ccccc}
        \toprule
        Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants \\
        \midrule
                                  & FastCLIP-v0                       & 31.47 (0.31)          & 34.86 (0.53)                & 24.55 (0.21) \\
                                  & FastCLIP-v1                 & 30.65 (0.11)          & 32.66 (0.12)                & 24.26 (0.06) \\
                                  & FastCLIP-v2                 & 30.95 (0.32)          & 33.71 (0.20)                & {\bf 24.94 (0.18)} \\
        \multirow{-4}{*}{Large}   & FastCLIP-v3                 & {\bf 31.60 (0.46)} & {\bf 34.88 (0.28)}       & 24.78 (0.28) \\
        \bottomrule
    \end{tabular}
    \label{tab:tau}
\vspace*{0.05in}

    \caption{Performance of different optimizers. Gap denotes improvements of AdamW on three metrics.}
    \begin{tabular}{cccccc}
        \toprule
        Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants              & \textit{Gap} \\
        \midrule
                                  & LAMB                        & 30.54 (0.24)          & 34.02 (0.26)                & 24.11 (0.21)          &  \\
        \multirow{-2}{*}{Large}   & AdamW                       & \textbf{31.60} (0.46) & \textbf{34.88} (0.28)       & \textbf{24.78} (0.28) & \multirow{-2}{*}{\textit{1.06, 0.86, 0.67}} \\
        \bottomrule
    \end{tabular}
    \label{tab:optimizer1}
\end{table}
\vspace*{0.1in}
}


==> floats/tab_components_medium.tex <==
{
% \renewcommand{\arraystretch}{1.1}
\definecolor{shaded}{gray}{0.93}
\begin{table}[t]
    \caption{Performance of different inner LR schedules. \colorbox{shaded}{Shaded} algorithms use the cosine schedule, while the others use the constant schedule. Improvement denotes the absolute difference between two algorithms on the three metrics. \(^*\): v3 (Const. \(\gamma\)) denotes FastCLIP-v3 with constant \(\gamma\) schedule.}
    % \begin{widepage}
        \centering
       \resizebox{0.9\columnwidth}{!}{ \begin{tabular}{cccccc}
            \toprule
            Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants              & \textit{Improvement} \\
            \midrule
                                    & SogCLR                          & 23.41 (0.34)          & 27.48 (0.24)                & 16.90 (0.01)          & \\
            \rowcolor{shaded}
            \cellcolor{white}        & FastCLIP-v1                     & \textbf{24.87} (0.13) & \textbf{29.28} (0.30)       & \textbf{18.86} (0.09) & \cellcolor{white} \multirow{-2}{*}{\textit{1.46, 1.80, 1.96}} \\
            \cline{2-6}
                                    & iSogCLR                         & 23.35 (0.63)          & 27.92 (0.34)                & 17.05 (0.14) &  \\
            \rowcolor{shaded}
            \cellcolor{white}        & FastCLIP-v2                     & \textbf{24.10} (0.34) & \textbf{29.32} (1.29)       & \textbf{18.52} (0.37) & \cellcolor{white} \multirow{-2}{*}{\textit{0.75, 1.40, 1.47}} \\
            \cline{2-6}
                                    & v3 (Const. \(\gamma\))\(^*\) & 23.60 (0.18)          & 27.68 (0.17)                & 17.33 (0.22) & \\
            \rowcolor{shaded}
            \cellcolor{white} \multirow{-6}{*}{Medium}& FastCLIP-v3                     & \textbf{24.76} (0.26) & \textbf{30.36} (0.18)       & \textbf{19.08} (0.16) & \cellcolor{white} \multirow{-2}{*}{\textit{1.16, 2.68, 1.75}} \\
            \bottomrule
        \end{tabular}}
    % \end{widepage}
    \label{tab:gamma}

\vspace*{0.05in}
    \centering
    \caption{Performance of different temperature parameter updates.}
    \begin{tabular}{ccccc}
        \toprule
        Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants \\
        \midrule
                                  & FastCLIP-v0                        & 24.71 (0.21)          & 30.36 (0.26)                & 17.50 (0.33) \\
                                  & FastCLIP-v1                 & {\bf 24.87 (0.13)}          & 29.28 (0.30)                & 18.86 (0.09) \\
                                  & FastCLIP-v2                 & 24.21 (0.76)          & 30.35 (0.47)                & 17.86 (0.21) \\
        \multirow{-3}{*}{Medium}  & FastCLIP-v3                 & 24.76 (0.26)          & {\bf 30.36 (0.18)}                & {\bf 19.08 (0.16)} \\
        \bottomrule
    \end{tabular}
    \label{tab:tau}
\vspace*{0.05in}

    \caption{Performance of different optimizers. Gap denotes improvements of AdamW on three metrics.}
    \begin{tabular}{cccccc}
        \toprule
        Setting                   & Algorithm                       & Datacomp              & Retrieval                   & IN \& Variants              & \textit{Gap} \\
        \midrule
                                  & LAMB                        & 22.63 (0.30)          & 24.87 (0.27)                & 16.43 (0.06)          &  \\
        \multirow{-2}{*}{Medium}  & AdamW                       & \textbf{24.76} (0.26) & \textbf{30.36} (0.18)       & \textbf{19.08} (0.16) & \multirow{-2}{*}{\textit{2.13, 5.49, 2.65}} \\
        \bottomrule
    \end{tabular}
    \label{tab:optimizer1}
\end{table}
\vspace*{0.1in}
}


==> sty_iclr25/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

